Uncertainty-Aware and Decoder-Aligned Learning for Video Summarization

Video summarization aims to produce a compact representation of a long video by selecting a subset of temporally important segments that best reflect human preferences. This task is inherently difficult due to strong annotation subjectivity and the reliance on discrete decoding procedures, such as temporal segmentation and knapsack-based selection, during evaluation. Most existing approaches either learn deterministic importance scores that overlook these characteristics or adopt complex generative models that increase training and inference cost. In this paper, we propose VASTSum, an uncertainty-aware and decoder-aligned learning framework for video summarization that addresses both challenges within a single-pass model. The proposed method predicts probabilistic frame-level importance scores using a variational formulation, enabling explicit modeling of uncertainty arising from multi-annotator supervision. To account for subjectivity, particularly under binary annotations, we employ a supervision strategy that encourages alignment with plausible human annotation modes rather than enforcing a single consensus target. Furthermore, we introduce a decoder-aligned regularization that promotes stability of knapsack-based summary selection, reducing sensitivity to small perturbations in predicted scores. We evaluate the proposed framework on the SumMe and TVSum benchmarks using standard rank-based metrics. Experimental results show consistent and competitive Kendall and Spearman correlations across multiple data splits, demonstrating improved robustness under annotation disagreement while maintaining efficient single-forward inference. These results indicate that explicitly modeling uncertainty and aligning learning objectives with the decoding stage provide a principled alternative to both deterministic and diffusion-based video summarization methods.

==> method.tex <==
\section{Problem Formulation}
\label{sec:problem}

Given a video $X \triangleq \{x_i\}_{i=1}^{N}$ with $N$ frames (or sampled timesteps), the goal of supervised video summarization is to predict frame-level importance such that a compact summary can be selected under a fixed length budget. A summary is represented by a binary indicator vector $y \in \{0,1\}^{N}$ satisfying
\begin{equation}
\sum_{i=1}^{N} y_i \leq S,
\end{equation}
where $S$ is determined by the evaluation protocol.

To reflect human subjectivity, standard benchmarks provide multiple annotations per video. Let $\mathcal{R}$ denote the set of annotators and let $s^{(r)} \in [0,1]^N$ denote the frame-level importance signal associated with annotator $r \in \mathcal{R}$ (continuous scores in TVSum and derived frame-level targets from user summaries in SumMe). A common deterministic formulation regresses a point estimate $s \in [0,1]^N$ toward an aggregated target such as the mean
\begin{equation}
\bar{s} \triangleq \frac{1}{|\mathcal{R}|}\sum_{r \in \mathcal{R}} s^{(r)},
\end{equation}
which collapses multi-annotator disagreement into a single supervision signal. In contrast, distributional formulations aim to capture multiple plausible summaries, but diffusion-based approaches typically require iterative sampling at inference.

Evaluation further depends on a discrete decoding stage that converts predicted scores into a binary summary. Specifically, scores are first pooled into temporally coherent keyshots using a segmentation procedure (e.g., KTS), and a subset of keyshots is then selected via knapsack optimization under the budget constraint. We denote this decoder by a deterministic operator
\begin{equation}
y = \mathcal{D}(s; X),
\end{equation}
which maps a score sequence $s$ (and video metadata such as segment lengths) to a binary summary. Since $\mathcal{D}$ is discrete, small perturbations in $s$ can change the selected keyshots, creating a mismatch between continuous training objectives and decoder-defined evaluation.

Our formulation addresses both properties, subjectivity and decoder sensitivity, within an efficient single-pass model. We predict importance as a conditional distribution $p_{\theta}(s \mid X)$, parameterized by a mean $\mu_{\theta}(X)$ and an uncertainty signal $\sigma_{\theta}(X)$, and train using the full set of annotations $\{s^{(r)}\}_{r \in \mathcal{R}}$ rather than a single collapsed target. To align learning with evaluation, we additionally encourage decoder stability by regularizing the consistency between $\mathcal{D}(s; X)$ and $\mathcal{D}(\tilde{s}; X)$ for perturbed scores $\tilde{s}$ sampled according to the predicted uncertainty. This problem formulation motivates the uncertainty-aware and decoder-aligned objectives introduced in the next section.

\subsection{Problem setup and inputs}
\label{sec:method_setup}

Given an untrimmed video, our goal is to produce a compact summary that preserves the essential content under a strict length budget.
We operate on pre-extracted frame representations and predict a frame-level importance signal that is subsequently decoded into a budgeted set of temporal segments.
Let
\begin{equation}
\mathbf{X} = \{\mathbf{x}_t \in \mathbb{R}^{D}\}_{t=1}^{T}
\end{equation}
denote the sequence of sampled frame features, where $T$ is the number of sampled timesteps and $D$ is the feature dimension.
In our implementation, $D=1024$ and the model consumes the sampled tensor extracted from the stored feature array.

The input is accompanied by temporal metadata that is used consistently during training and inference.
First, a sampling index sequence
\begin{equation}
\mathbf{p} = \{p_t\}_{t=1}^{T}, \qquad 0 \le p_1 < \cdots < p_T < N,
\end{equation}
maps each sampled timestep to its location on the original timeline of $N$ frames.
Second, a change-point partition of the original timeline is provided by Kernel Temporal Segmentation, represented as
\begin{equation}
\mathbf{C} = \{(c_k^{\mathrm{start}}, c_k^{\mathrm{end}})\}_{k=1}^{M},
\end{equation}
where the segments are disjoint and cover the video in temporal order.
This partition defines $M$ contiguous segments and provides the structural units used by both the scorer and the budgeted decoder.

We seek a binary summary on the original timeline,
\begin{equation}
\mathbf{y} \in \{0,1\}^{N},
\end{equation}
subject to a length constraint
\begin{equation}
\sum_{n=1}^{N} y_n \le \rho N,
\end{equation}
where $\rho=0.15$ is the standard evaluation budget.
Rather than predicting $\mathbf{y}$ directly, we learn a scoring function that produces an importance signal on the sampled timeline and decode it into a valid summary through a deterministic budgeted selection step.

Two empirical properties motivate our design.
The first is that supervision is inherently subjective: benchmarks provide multiple user annotations that may disagree on what constitutes an essential moment.
The second is that summary generation involves discrete budgeted selection: small variations in predicted scores can lead to different knapsack solutions, which changes the final summary.
Accordingly, our method is built around a probabilistic scoring head that can represent uncertainty in frame importance and a training objective that regularizes the score geometry to support stable budgeted selection.

\subsection{Segmentation-aware indexing and hierarchical structure}
\label{sec:method_segmap}

We use the temporal partition produced by KTS as an explicit structural prior.
The partition is defined on the original timeline of length $N$ by the ordered set of change points
\begin{equation}
\mathbf{C}=\{(c_k^{\mathrm{start}},c_k^{\mathrm{end}})\}_{k=1}^{M},
\end{equation}
where segments are contiguous, disjoint, and cover the video.
The model operates on a sampled timeline of length $T$ determined by the sampling indices
\begin{equation}
\mathbf{p}=\{p_t\}_{t=1}^{T}, \qquad 0 \le p_1 < \cdots < p_T < N.
\end{equation}
To connect these two temporal representations, we define a deterministic mapping from each sampled timestep to a segment identity.

For each sampled index $p_t$, we assign a segment id
\begin{equation}
s_t = k \quad \Longleftrightarrow \quad c_k^{\mathrm{start}} \le p_t \le c_k^{\mathrm{end}},
\qquad t=1,\dots,T,
\end{equation}
which yields the segment-id sequence
\begin{equation}
\mathbf{s}=\{s_t\}_{t=1}^{T}, \qquad s_t\in\{1,\dots,M\}.
\end{equation}
This mapping induces segment-specific index sets on the sampled timeline,
\begin{equation}
\mathcal{I}_k = \{t \in \{1,\dots,T\} \mid s_t = k\},
\end{equation}
and segment lengths on the original timeline,
\begin{equation}
\ell_k = c_k^{\mathrm{end}} - c_k^{\mathrm{start}} + 1, 
\qquad k=1,\dots,M.
\end{equation}
When needed, we also use the number of sampled frames assigned to each segment,
\begin{equation}
n_k = |\mathcal{I}_k|.
\end{equation}

This hierarchical indexing plays two roles in the proposed method.
First, it provides a compact set of temporal units for global reasoning, enabling long-range interactions to be modeled over $M$ segment tokens rather than over $T$ frames.
Second, it establishes the consistent interface between the frame-level scorer and the budgeted decoder: frame-level predictions can be aggregated within each segment using $\{\mathcal{I}_k\}$, while the budget constraint is enforced using segment lengths $\{\ell_k\}$ on the original timeline.

\subsection{Hierarchical segment-context scoring network}
\label{sec:method_model}

The scoring network maps sampled frame features to a frame-level importance signal while incorporating long-range temporal structure induced by the change-point partition.
The method follows a hierarchical design: it first forms a compact sequence of segment representations, performs global reasoning over segments using a Transformer encoder, and then injects the resulting segment context back into frame-level tokens through a learned fusion mechanism.
This preserves frame resolution for scoring, while performing global interaction over a much shorter sequence since typically $M \ll T$.

We begin by projecting frame features to a model space of dimension $d$ and adding a learnable temporal positional embedding:
\begin{equation}
\mathbf{h}_t^{(0)} = \mathrm{LN}(\mathbf{W}_{\mathrm{in}}\mathbf{x}_t + \mathbf{b}_{\mathrm{in}}) + \boldsymbol{\phi}_t,
\qquad t=1,\dots,T,
\end{equation}
where $\boldsymbol{\phi}_t \in \mathbb{R}^{d}$ encodes the order of sampled timesteps.

The segment-id sequence $\mathbf{s}=\{s_t\}_{t=1}^{T}$ defines a partition of sampled indices into sets
$\mathcal{I}_k = \{t \mid s_t = k\}$.
We form one segment token per segment by mean pooling the projected frame tokens:
\begin{equation}
\mathbf{z}_k^{(0)} = \frac{1}{|\mathcal{I}_k|}\sum_{t\in\mathcal{I}_k} \mathbf{h}_t^{(0)},
\qquad k=1,\dots,M.
\end{equation}
Stacking these tokens yields $\mathbf{Z}^{(0)} \in \mathbb{R}^{M\times d}$.

We model dependencies among segments using a stack of $L$ Transformer encoder layers in a pre-normalized form.
Let $\mathbf{Z}^{(\ell)}$ be the segment token matrix at layer $\ell$.
Each layer applies multi-head self-attention followed by a position-wise feed-forward block:
\begin{align}
\mathbf{U}^{(\ell)} &= \mathbf{Z}^{(\ell)} + \mathrm{MHA}\!\left(\mathrm{LN}\!\left(\mathbf{Z}^{(\ell)}\right)\right), \\
\mathbf{Z}^{(\ell+1)} &= \mathbf{U}^{(\ell)} + \mathrm{FFN}\!\left(\mathrm{LN}\!\left(\mathbf{U}^{(\ell)}\right)\right),
\qquad \ell=0,\dots,L-1.
\end{align}

Multi-head attention is defined by $H$ heads with per-head dimension $d_h=d/H$.
For head $h$, we compute
\begin{equation}
\mathbf{Q}_h = \mathbf{Z}\mathbf{W}_h^{Q},\quad
\mathbf{K}_h = \mathbf{Z}\mathbf{W}_h^{K},\quad
\mathbf{V}_h = \mathbf{Z}\mathbf{W}_h^{V},
\end{equation}
where $\mathbf{W}_h^{Q},\mathbf{W}_h^{K},\mathbf{W}_h^{V}\in\mathbb{R}^{d\times d_h}$.
Attention for head $h$ is
\begin{equation}
\mathrm{Attn}_h(\mathbf{Z}) =
\mathrm{softmax}\!\left(\frac{\mathbf{Q}_h\mathbf{K}_h^{\top}}{\sqrt{d_h}}\right)\mathbf{V}_h
\in \mathbb{R}^{M\times d_h}.
\end{equation}
The multi-head output is obtained by concatenation and output projection:
\begin{equation}
\mathrm{MHA}(\mathbf{Z}) =
\big[\mathrm{Attn}_1(\mathbf{Z});\dots;\mathrm{Attn}_H(\mathbf{Z})\big]\mathbf{W}^{O},
\end{equation}
with $\mathbf{W}^{O}\in\mathbb{R}^{d\times d}$.
The feed-forward network is applied token-wise:
\begin{equation}
\mathrm{FFN}(\mathbf{z}) =
\mathbf{W}_2\,\mathrm{GELU}(\mathbf{W}_1\mathbf{z} + \mathbf{b}_1) + \mathbf{b}_2.
\end{equation}
After $L$ layers, we obtain contextualized segment tokens
$\mathbf{C}=\mathbf{Z}^{(L)}\in\mathbb{R}^{M\times d}$.

To return to frame resolution, each frame retrieves the context of its assigned segment:
\begin{equation}
\mathbf{g}_t = \mathbf{c}_{s_t}\in\mathbb{R}^{d}, \qquad t=1,\dots,T.
\end{equation}
We fuse local frame information with global segment context using a learned gate:
\begin{align}
\boldsymbol{\alpha}_t &= \sigma\!\left(\mathbf{W}_g
\begin{bmatrix}
\mathbf{h}_t^{(0)} \\ \mathbf{g}_t
\end{bmatrix}
+ \mathbf{b}_g\right)\in (0,1)^{d},\\
\tilde{\mathbf{h}}_t &= \mathrm{LN}\!\left(\mathbf{h}_t^{(0)} + \boldsymbol{\alpha}_t \odot \mathbf{g}_t\right).
\end{align}
This fusion allows the model to modulate, at each timestep and channel, how strongly segment-level context should influence the frame-level representation.

Finally, we refine the fused frame sequence to capture local temporal patterns.
Let $\tilde{\mathbf{H}}\in\mathbb{R}^{T\times d}$ stack the fused tokens.
We apply a residual temporal refinement operator:
\begin{equation}
\hat{\mathbf{H}} = \tilde{\mathbf{H}} + \Psi(\tilde{\mathbf{H}}),
\end{equation}
where $\Psi$ is a lightweight temporal module implemented with depthwise separable temporal convolutions and pointwise mixing.
The refined frame tokens $\hat{\mathbf{H}}$ are then passed to the probabilistic head in Sec.~\ref{sec:method_probhead} to produce per-frame importance predictions.

\subsection{Dataset-aligned score usage at inference}
\label{sec:method_infer_use}

At inference time, the scoring network produces a deterministic importance signal on the sampled timeline.
Specifically, we use the posterior mean in the probabilistic head, yielding a per-frame score sequence
\begin{equation}
\boldsymbol{\mu} = \{\mu_t\}_{t=1}^{T}, \qquad \mu_t \in \mathbb{R},
\end{equation}
which serves as the sole input to the downstream budgeted decoder.

Although the architecture is shared across datasets, the supervision formats differ.
Accordingly, we employ a dataset-aligned calibration step that maps the predicted mean scores to the form required by each benchmark protocol.

For datasets that provide continuous frame-level importance annotations, the output $\mu_t$ is interpreted directly as a continuous importance estimate.
In this case, the decoder operates on the real-valued score sequence $\boldsymbol{\mu}$.

For datasets whose supervision is expressed as binary user summaries, we convert the predicted mean scores into probabilities through temperature scaling:
\begin{equation}
\tilde{\mu}_t = \sigma\!\left(\frac{\mu_t}{\tau}\right),
\qquad t=1,\dots,T,
\end{equation}
where $\sigma(\cdot)$ denotes the logistic sigmoid and $\tau>0$ is a fixed temperature.
This transformation controls the sharpness of the probability outputs and yields a calibrated score sequence
$\tilde{\boldsymbol{\mu}}=\{\tilde{\mu}_t\}_{t=1}^{T}$.
The subsequent decoding step is identical across datasets and depends only on the provided change points and the resulting score sequence on the sampled timeline.

\subsection{Budgeted decoding to generate the final summary}
\label{sec:method_decode}

The final summary is obtained by solving a budgeted segment selection problem defined on the change-point partition.
The decoder takes as input the predicted score sequence on the sampled timeline, the sampling indices $\mathbf{p}$, and the change points $\mathbf{C}$ on the original timeline.
It outputs a binary indicator vector on the original timeline,
\begin{equation}
\mathbf{y} \in \{0,1\}^{N},
\end{equation}
that satisfies the length budget.

Let $\mathbf{s}=\{s_t\}_{t=1}^{T}$ be the segment-id sequence induced by $\mathbf{C}$ and $\mathbf{p}$ as defined in Sec.~\ref{sec:method_segmap}.
We first construct a dense score sequence on the original timeline.
Define $\mathbf{f}\in\mathbb{R}^{N}$ such that for each sampled timestep $t$ the score is assigned to the interval between consecutive picks:
\begin{equation}
f_n = \mu_t \quad \text{for} \quad n \in [p_t,\, p_{t+1}),
\qquad t=1,\dots,T-1,
\end{equation}
and for the final interval,
\begin{equation}
f_n = \mu_T \quad \text{for} \quad n \in [p_T,\, N).
\end{equation}
This expansion yields a frame-level score sequence aligned with the original timeline.

We then define one value and one cost per segment.
For each segment $k\in\{1,\dots,M\}$, the cost is its length in frames,
\begin{equation}
w_k = \ell_k = c_k^{\mathrm{end}} - c_k^{\mathrm{start}} + 1,
\end{equation}
and the value is the mean score within that segment,
\begin{equation}
v_k = \frac{1}{w_k}\sum_{n=c_k^{\mathrm{start}}}^{c_k^{\mathrm{end}}} f_n.
\end{equation}
Given a fixed budget ratio $\rho=0.15$, the decoder selects a subset of segments by solving the 0/1 knapsack problem
\begin{equation}
\max_{\mathbf{u}\in\{0,1\}^{M}} \ \sum_{k=1}^{M} u_k v_k
\quad \text{s.t.} \quad \sum_{k=1}^{M} u_k w_k \le \rho N.
\label{eq:knapsack}
\end{equation}
The selected segments are then expanded to a binary summary on the original timeline:
\begin{equation}
y_n =
\begin{cases}
1, & \text{if } \exists k \text{ such that } u_k=1 \text{ and } c_k^{\mathrm{start}}\le n \le c_k^{\mathrm{end}},\\
0, & \text{otherwise.}
\end{cases}
\end{equation}
This produces a valid summary under the required length budget, and it is the representation used for evaluation on summary-based benchmarks.

\subsection{Training objectives and optimization}
\label{sec:method_train}

The model is trained end to end to predict an importance signal on the sampled timeline, while remaining compatible with the discrete, budgeted decoder in Sec.~\ref{sec:method_decode}.
Because supervision differs across benchmarks, we use dataset-aligned likelihood terms and share a common set of regularizers that enforce temporal ordering, control the latent distribution, and improve robustness of budgeted selection.

\paragraph{TVSum supervision.}
TVSum provides continuous frame-level importance scores from multiple users.
Let $\{y_{u,t}\}_{u=1}^{U}$ denote the annotator scores at sampled timestep $t$.
The probabilistic head defines a heteroscedastic Gaussian model with mean $\mu_t$ and variance $v_t=\exp(\log v_t)$.
We minimize the multi-annotator Gaussian negative log-likelihood
\begin{equation}
\mathcal{L}_{\mathrm{tv}}
=
\frac{1}{UT}\sum_{u=1}^{U}\sum_{t=1}^{T}
\frac{1}{2}
\left(
\log v_t
+
\frac{(y_{u,t}-\mu_t)^2}{v_t+\epsilon}
\right),
\label{eq:tvsum_nll}
\end{equation}
where $\epsilon$ is a small constant for numerical stability.
This objective encourages accurate means while allowing the variance to represent disagreement and ambiguity.

\paragraph{SumMe supervision.}
SumMe provides binary user summaries.
Let $a_{u,t}\in\{0,1\}$ denote the binary label at sampled timestep $t$ from annotator $u$.
We convert the predicted mean scores to probabilities using temperature scaling,
\begin{equation}
p_t = \sigma\!\left(\frac{\mu_t}{T_s}\right),
\label{eq:summe_prob}
\end{equation}
where $T_s>0$ is fixed.
For each annotator we define a frame-level binary cross-entropy,
\begin{equation}
\mathrm{BCE}_u
=
\frac{1}{T}\sum_{t=1}^{T}
\left(
-a_{u,t}\log p_t
-(1-a_{u,t})\log(1-p_t)
\right).
\label{eq:summe_bce}
\end{equation}
Instead of averaging annotators, we use a soft-min aggregation that emphasizes matching at least one plausible annotator:
\begin{equation}
\mathcal{L}_{\mathrm{sm}}
=
-\tau_{\mathrm{sm}}
\log
\sum_{u=1}^{U}
\exp\!\left(-\frac{\mathrm{BCE}_u}{\tau_{\mathrm{sm}}}\right),
\label{eq:softmin_bce}
\end{equation}
where $\tau_{\mathrm{sm}}>0$ controls the softness of the minimum.

\paragraph{Pairwise ranking regularization.}
To encourage correct relative ordering of importance, we add a lightweight pairwise hinge loss.
Given a target sequence $r_t$ on the sampled timeline, we sample index pairs $(i,j)$ and keep those with $r_i>r_j$.
For predictions $q_t$ and margin $m>0$, the ranking loss is
\begin{equation}
\mathcal{L}_{\mathrm{rank}}
=
\mathbb{E}_{(i,j):\, r_i>r_j}
\left[
\max\!\big(0,\ m-(q_i-q_j)\big)
\right].
\label{eq:rank_hinge}
\end{equation}
For TVSum we set $q_t=\mu_t$ and $r_t=\frac{1}{U}\sum_u y_{u,t}$.
For SumMe we set $q_t=p_t$ and choose $r_t=a_{u^\star,t}$ from the annotator $u^\star$ that minimizes $\mathrm{BCE}_u$ in \eqref{eq:summe_bce}.

\paragraph{Latent regularization.}
The probabilistic head includes a latent variable with posterior
$q_{\theta}(\mathbf{z}_t\mid \hat{\mathbf{h}}_t)=\mathcal{N}(\boldsymbol{\mu}_{z,t},\mathrm{diag}(\boldsymbol{\sigma}^2_{z,t}))$
and prior $p(\mathbf{z}_t)=\mathcal{N}(\mathbf{0},\mathbf{I})$.
We regularize with the standard KL divergence
\begin{equation}
\mathcal{L}_{\mathrm{kl}}
=
\frac{1}{T}\sum_{t=1}^{T}
\mathrm{KL}\!\left(
q_{\theta}(\mathbf{z}_t\mid \hat{\mathbf{h}}_t)\ \|\ p(\mathbf{z}_t)
\right).
\label{eq:kl}
\end{equation}

\paragraph{Knapsack stability regularization.}
Budgeted decoding is sensitive to small perturbations in segment values.
To align training with the discrete selection step, we apply a stability regularizer at the segment level.
Let $s_k$ be the pooled score of segment $k$ obtained by averaging the frame-level signal within that segment on the sampled timeline.
For TVSum we pool $\mu_t$, and for SumMe we pool $p_t$.
Let $\mathbf{z}^{(0)}\in\{0,1\}^{M}$ be the knapsack selection computed from $\{s_k\}$ under the budget in \eqref{eq:knapsack}.
We then draw $R$ perturbations $\boldsymbol{\epsilon}^{(r)}\sim\mathcal{N}(\mathbf{0},\sigma^2\mathbf{I})$ and compute selections
$\mathbf{z}^{(r)}$ from $\{s_k+\epsilon^{(r)}_k\}$.
Define the selection frequency $\bar{z}_k=\frac{1}{R}\sum_r z_k^{(r)}$ and the unstable set
\begin{equation}
\mathcal{U}=\{k \mid 0<\bar{z}_k<1\}.
\end{equation}
Let $\mathcal{S}=\{k \mid z_k^{(0)}=1\}$ and $\bar{\mathcal{S}}=\{k \mid z_k^{(0)}=0\}$ denote selected and unselected segments under the base solution.
With a margin $m_s>0$, we impose separation constraints for unstable segments:
\begin{align}
\mathcal{L}_{\mathrm{stab}}
&=
\frac{1}{|\mathcal{U}\cap\mathcal{S}|}\sum_{k\in\mathcal{U}\cap\mathcal{S}}
\max\!\Big(0,\ m_s-\big(s_k-\max_{j\in\bar{\mathcal{S}}} s_j\big)\Big)
\nonumber\\
&\quad+
\frac{1}{|\mathcal{U}\cap\bar{\mathcal{S}}|}\sum_{k\in\mathcal{U}\cap\bar{\mathcal{S}}}
\max\!\Big(0,\ m_s-\big(\min_{i\in\mathcal{S}} s_i-s_k\big)\Big),
\label{eq:stab_margin}
\end{align}
with the convention that empty sums contribute zero.
This term does not differentiate through the knapsack solver; instead, it uses solver outputs to identify unstable segments and then shapes the score margins with respect to the current, differentiable segment scores.

\paragraph{Overall objective and optimization.}
Let $\mathcal{L}_{\mathrm{main}}$ denote the dataset likelihood, using $\mathcal{L}_{\mathrm{tv}}$ for TVSum and $\mathcal{L}_{\mathrm{sm}}$ for SumMe.
The full training loss is
\begin{equation}
\mathcal{L}
=
\mathcal{L}_{\mathrm{main}}
+
\lambda_{\mathrm{rank}}(e)\,\mathcal{L}_{\mathrm{rank}}
+
\lambda_{\mathrm{stab}}(e)\,\mathcal{L}_{\mathrm{stab}}
+
\lambda_{\mathrm{kl}}(e)\,\mathcal{L}_{\mathrm{kl}},
\label{eq:full_loss}
\end{equation}
where $\lambda_{\mathrm{rank}}(e)$, $\lambda_{\mathrm{stab}}(e)$, and $\lambda_{\mathrm{kl}}(e)$ follow linear warm-up schedules over the first epochs of training.
We optimize \eqref{eq:full_loss} with AdamW, apply gradient-norm clipping, and use minibatch accumulation over videos to match the configured effective batch size.
